Safe Exploration for Interactive Machine Learning

In Interactive Machine Learning (IML), we iteratively make decisions and obtain noisy observations of an unknown function. While IML methods, e.g., Bayesian optimization and active learning, have been successful in applications, on real-world systems they must provably avoid unsafe decisions. To this end, safe IML algorithms must carefully learn about a priori unknown constraints without making unsafe decisions. Existing algorithms for this problem learn about the safety of all decisions to ensure convergence. This is sample-inefficient, as it explores decisions that are not relevant for the original IML objective. In this paper, we introduce a novel framework that renders any existing unsafe IML algorithm safe. Our method works as an add-on that takes suggested decisions as input and exploits regularity assumptions in terms of a Gaussian process prior in order to efficiently learn about their safety. As a result, we only explore the safe set when necessary for the IML problem. We apply our framework to safe Bayesian optimization and to safe exploration in deterministic Markov Decision Processes (MDP), which have been analyzed separately before. Our method outperforms other algorithms empirically.

==> proofs/6-unused_lemmas.tex <==
\begin{restatable}{lemma}{NonIncreasingSopt}
\label{lem:NonIncreasingSopt}
    For any $t\geq 1$, $\Sopt_0\supseteq \Sopt_t \supseteq \Sopt_{t+1}$ and $\Shato_0\supseteq \Shato_t \supseteq \Shato_{t+1}$ with probability at least $1-\delta$.
\end{restatable}
\begin{proof}
    Consider $\s \in \Sopt_t$ for any $t\geq 0$.
    Trivially, we have $\s \in \Sopt_0$, since $\Sopt_0 = \mathcal{D}$ by initialization. Moreover, for $t \geq 1$ we have $\Sopt_t \supseteq \Sopt_{t+1}$ by \cref{lem:monotonicity}. Similarly, we can say $\Shato_0 \supseteq \Shato_t$ for all $t \geq 1$. To show $\Shato_t \supseteq \Shato_{t+1}$, we proceed by induction. We use $\Shato_t \supseteq \Shato_{t-1}$ as induction hypothesis, which trivially holds for $t = 1$ for the reasons above. Thererfore, we can say
    \begin{equation*}
        \Shato_{t+1} = \Sopt_{t+1} \cap \Rerg(\Sopt_{t+1}, \Shato_t) \subseteq \Sopt_{t} \cap \Rerg(\Sopt_{t}, \Shato_{t-1}) = \Shato_{t},  
    \end{equation*}
    by the inductive hypothesis and \cref{lem:RergSubset}.
\end{proof}
%
%
%
\begin{restatable}{lemma}{SpessInSopt}
    \label{lem:SpessInSopt}
    For any $t\geq 0$, $\Spess_t \subseteq \Sopt_t$ with probability at least $1 - \delta$.
\end{restatable}
\begin{proof}
    For $t=0$, it holds by initialization. For $t \geq 1$, we have that $\s \in \Spess_t$ implies that $\exists \z \in \Spess_{t-1}$ such that:
    \begin{align*}
        & l_t(\z) - Ld(\z, \s) \geq 0,  \\
        & q(\z) - Ld(\z, \s) \geq 0,  \tag*{by \cref{thm:beta}} \\ 
        & q(\s) \geq 0, \tag*{by Lipschitz continuity}\\
        & u_t(\s) \geq 0, \tag*{by \cref{thm:beta}}.
    \end{align*}
\end{proof}
%
%
%
\begin{restatable}{lemma}{ShatpInShato}
\label{lem:ShatpInShato}
    For any $t\geq 0$, $\Shatp_t \subseteq \Shato_t$ with probability at least $1 - \delta$.
\end{restatable}
\begin{proof}
    Let us proceed by induction. For the case $t=0$, it holds trivially by initialization. Therefore, our inductive assumption is $\Shatp_{t-1} \subseteq \Shato_{t-1}$. This allows us to write, 
    \begin{equation*}
        \Shatp_t = \Spess_t \cap \Rerg(\Spess_t, \Shatp_{t-1}) \subseteq\Sopt_t \cap R^{\mathrm{ergodic}}(\Sopt_t,\Shato_{t-1}) = \Shato_t,
    \end{equation*}
    by \cref{lem:SpessInSopt,lem:RergSubset}, and this completes the induction step.
\end{proof}
%
%
%
\begin{restatable}{lemma}{RepsShatpSubsetShato}
\label{lem:RepsShatpSubsetShato}
    For every $t \geq 0$, it holds $R_\epsilon(\Shatp_t) \subseteq \Shato_t$.
\end{restatable}
\begin{proof}
    Consider $\s \in \Rsafe_\epsilon (\Shatp_t)$, we know that $\exists \z \in \Shatp_t$ such that $q(\z) - \epsilon - Ld(\s, \z) \geq 0$, which implies that $q(\s) \geq 0$, which means, due to \cref{thm:beta},  that $u_t(\s) \geq 0$ and $\s \in \Sopt_t$. This shows that $\Rsafe_\epsilon(\Shatp_t) \subseteq \Sopt_t$. Moreover, we know that $\Shatp_t \subseteq \Shato_t \subseteq \Shato_{t-1}$ due to \cref{lem:ShatpInShato,lem:NonIncreasingSopt}. Therefore, we can use \cref{lem:RergSubset} to say
    \begin{equation*}
        R_\epsilon(\Shatp_t) = \Rsafe_\epsilon (\Shatp_t) \cap \Rerg (\Rsafe_\epsilon(\Shatp_t), \Shatp_t) \subseteq  \Sopt_t \cap R^{\mathrm{ergodic}}(\Sopt_t,\Shato_{t-1}) = \Shato_t.
    \end{equation*}
\end{proof}

\begin{restatable}{lemma}{StopExploration}
\label{lem:StopExploration}
There exists $\hat{t} \leq t^*$ such that $w_{\hat{t}}(\s)\leq \epsilon,~\forall \s \in g_{\hat{t}} (\hat{S}_{\hat{t}}, S_{\hat{t}})$ with probability at least $1 - \delta$.
\end{restatable}
\begin{proof}
In order to show that this holds true, we can show that there exist $\hat{t}\leq t^*$ such that $\hat{S}_{\hat{t}}=\hat{S}_{|\hat{S}_{\hat{t}}|T_{t^*}}$ and apply \cref{lem:UncertaintyInExpanders}. For the sake of contradiction, assume that for all $t\leq t^*$, it holds that $\hat{S}_{t}\subset\hat{S}_{|\hat{S}_{t}|T_{t^*}}$. Similarly to \cref{lem:ContainREpsilon}, for all $k \geq 1$ define $t_k = |\hat{S}_{t_{k-1}}|T_{t^*}$ with $t_0 = 0$. Our assumption implies that $\hat{S}_0 \subset \hat{S}_{t_1} \subset \hat{S}_{t_2}\subset \cdots$.
In general this means that $|\hat{S}_{t_k}| \geq |\hat{S}_0| + k$ for all $k \geq 1$. In particular if we set $k=|\Rbar_0(S_0) \setminus S_0| + 1$ we get that $|\hat{S}_{t_k}| \geq |\hat{S}_0| + |\Rbar_0(S_0) \setminus S_0| + 1= |\Rbar_0(S_0)| + 1 > |\Rbar_0(S_0)|$. This is a contradiction because of \cref{lem:Superset}.
\end{proof}
%
%
%
\begin{restatable}{lemma}{RemovalCondition}
\label{lem:RemovalCondition}
    If $g_t(W^\epsilon_t, \Shato_t \setminus \Spess_t) = \emptyset$ and $\Shatp_t = \Shatp_{t-1}$, then $\Rbar_\epsilon(S_0) \subseteq \Shatp_t$.
\end{restatable}
%
\begin{proof}
    Assume that this is not the case and $\Rbar_\epsilon(S_0) \setminus \Shatp_t \neq \emptyset$. Due to \cref{lem:ShortTermExploration}, we there exists $\s \in R_\epsilon(\Shatp_t) \setminus \Shatp_t$. At this point, we distinguish two cases: if $\s \in R_\epsilon(\Shatp_t) \setminus \Spess_t$ or $\s \in R_\epsilon(\Shatp_t) \cap \Spess_t \setminus \Shatp_t$. We start with the first case. Since $\s \in R_\epsilon(\Shatp_t) \setminus \Spess_t$ and $\Shatp_t = \Shatp_{t-1}$, we know that $\s \in \Rsafe_\epsilon(\Shatp_{t-1}) \setminus \Spess_t$ and, therefore, there exists $\z \in \Shatp_t = \Shatp_{t-1}$ such that 
    \begin{equation}
        q(\z) - \epsilon - Ld(\s, \z) >0. \label{eq:RemovalConditioEq1}   
    \end{equation}
    We further distinguish two cases: if $u_t(\z) - l_t(\z) > \epsilon$ or $u_t(\z) - l_t(\z) \leq \epsilon$. In  case $u_t(\z) - l_t(\z) > \epsilon$, we use \cref{eq:RemovalConditioEq1,thm:beta,lem:RepsShatpSubsetShato} to conclude that $\z \in g_t(W^\epsilon_t, \Shato_t \setminus \Spess_t)$, which is a contradiction. Otherwise, if $u_t(\z) - l_t(\z) \leq \epsilon$, we use \cref{eq:RemovalConditioEq1,thm:beta} to conclude that $l_t(\z) - Ld(\s, \z) \geq 0$. Since $\z \in \Shatp_{t-1}$, this allows us to say $\s \in \Spess_t$, which is a contradiction. We now turn to the second case of our initial distinction, $\s \in R_\epsilon(\Shatp_t) \cap \Spess_t \setminus \Shatp_t$. We aim to reach the following contradiction $\s \in \Shatp_t$. We already know that $\s \in \Spess_t$ and $\s \in R_\epsilon(\Shatp_t)$, which implies that $\s \in \Rerg (\Rsafe_\epsilon (\Shatp_t), \Shatp_t)$. Since we have by assumption that $\Shatp_t = \Shatp_{t-1}$, all we need to prove to reach the contradiction is $\Rsafe_\epsilon (\Shatp_t) = \Rsafe_\epsilon (\Shatp_{t-1}) \subseteq \Spess_t$ and apply \cref{lem:RergSubset}. However, we have already proved in the first of the two cases that we distinguished that indeed $\Rsafe_\epsilon (\Shatp_{t-1}) \subseteq \Spess_t$. Therefore, $\s \in \Spess_t$ and $\s \in \Rerg (\Rsafe_\epsilon (\Shatp_t), \Shatp_t) \subseteq \Rerg (\Spess_t, \Shatp_{t-1})$. This allows us to say $\s \in \Shatp_t$, which is a contradiction.
\end{proof}


==> sections/3-algorithm_old.tex <==
%!TEX root = ../root.tex

\section{Goal-oriented Safe Exploration (\goose)} 
\label{sec:Algorithm}

In this section, we present our algorithm, \goose. We do not propose a new \textit{safe} algorithm for a specific \gls{IML} setting, but instead exploit that, for specific \textit{IML} problems high-performance, \textit{unsafe} algorithms already exist. We treat any such \textit{unsafe} algorithm as an \gls{IML} oracle $\mathcal{O}_k(S)$, which, given a domain $S$ and $k-1$ observations of $f$, suggests a new decision $\goal_k \in S$, see \cref{fig:alg_explanation} (blue shaded).

\goose can extend any such \textit{unsafe} \gls{IML} algorithm to the safety-constrained setting. Thus, we effectively leave the problem of querying $f$ to the oracle and only consider safety. Given an \textit{unsafe} oracle decision $\goal_k$, \goose only evaluates $f(\goal_k)$ if the decisions $\goal_k$ is known to be safe. Otherwise, it \textit{safely learns} about $q(\goal_k)$ by safely and efficiently collecting observations $q(\s_t)$. Eventually it either learns that $\goal_k$ is safe and allows the oracle to evaluate $f(\goal_k)$, or the decision is unsafe, in which case the decision set of the oracle is restricted and a new decision is queried, see \cref{fig:alg_explanation}.

Previous approaches treat the expansion of the safe set as a proxy-objective to provide completeness guarantees. Instead, \goose employs goal-directed exploration scheme with a novel theoretical analysis that shifts the focus from greedily reducing the uncertainty \textit{inside} the safe set to learning about the safety of decisions \textit{outside} of it. This scheme retains the worst-case guarantees of existing methods, but is significantly more sample-efficient in practice. Moreover, \goose encompasses existing methods for this problem. % by using an uninformative, uncertainty-driven heuristic.
%
We now describe the detailed steps of \goose in \cref{alg:goose}.

\paragraph{Optimistic oracle}
%
The \gls{IML} oracle $\mathcal{O}(S)$ suggests  decisions $\goal_k \in S$ to evaluate within a given subset $S$ of $\mathcal{D}$. To make the oracle more efficient, we use the posterior belief over the safety constraint $q$ to eliminate decisions that are known to be unsafe with high probability. Analogously to the safe set, we define $\Sopt_t$ in \cref{alg:goose:line:safe_set_opt} of \cref{alg:goose} as the set of decisions that optimistically satisfy the safety constraints according to the GP confidence intervals from \cref{sec:ProblemStatement} and apply the ergodicity operator to obtain an optimistic safe set $\Shato_t$ in \cref{alg:goose:line:intersect_sopt_with_ergodic}. The set $\Shato_t$ eliminates any decisions from $\mathcal{D}$ that are known to be unsafe in the short- or long-term, or are not safely reachable.
%
The oracle uses this set in \cref{alg:goose:line:oracle_suggestion} to suggest a potentially unsafe, candidate decision $\goal_k = \mathcal{O}(\Shato_t)$.

\paragraph{Safe evaluation}
%
We determine safety of the suggestion $\goal_k$ as \citet{turchetta2016safe} and construct the set $\Shatp_t$ of decisions that are safe to evaluate in \cref{alg:goose:line:safe_set_pess,alg:goose:line:intersect_spess_with_ergodic}, see \cref{sec:ProblemStatement}. 
%
If we know that $\goal_k$ is safe to evaluate, i.e., $\goal_k \in \Shatp_t$, then the oracle obtains a noisy observation of $f(\goal_k)$ in \cref{alg:goose:line:evaluate_suggestion}. Otherwise \goose proceeds to safely learn about the safety of $\goal_k$ using a safe expansion strategy in lines \crefrange{alg:goose:line:while_unsafe}{alg:goose:line:remove_unsafe_oracle_suggestion} that we outline in the following. If, after this routine, we conclude that $\goal_k$ is safe, then the oracle obtains the desired observation $f(\goal_k)$. Otherwise we remove it from the oracle's decision set $\Shato_t$ and query a new decision from the oracle in \cref{alg:goose:line:remove_unsafe_oracle_suggestion}, without evaluating $f(\goal_k)$.


\begin{figure*}
\noindent
\begin{minipage}[t]{0.53\textwidth}
\centering
\begin{algorithm}[H]
\caption{\goose}
\label{alg:SMDP_priority}
\label{alg:goose}
\begin{algorithmic}[1]
  \algsetup{indent=1em}
  \STATE \textbf{Inputs:} \parbox[t]{0.75\linewidth}{%
          %Kernels $k_f(\cdot,\cdot),~ k_q(\cdot,\cdot)$, %\newline
          Lipschitz constant $L$, %\newline
          Seed $S_0$, Graph $\mathcal{G}$, Oracle $O$, Accuracy $\epsilon$.
            }
    \STATE $\Spess_0 = \Shatp_0 \gets S_0$, $\Sopt_0 = \Shato_0 \gets \mathcal{D}, t \gets 0$
    %
    \FOR{$k=1,2,\ldots$}
        %
        \STATE $\goal_k \gets O(\Shato_t)$
        \label{alg:goose:line:oracle_suggestion}
        %
        \WHILE{$\goal_k \not \in \Shatp_t$}
        \label{alg:goose:line:while_unsafe}
            \STATE $\s_t \gets \mathrm{SE}(\Shato_t, \Shatp_t, \Spess_t, \mathcal{G},\goal_t)$, $t\gets t+1$
            \label{alg:goose:line:safe_exploration}
            %
            \STATE
            \begin{varwidth}[t]{\linewidth}
                $\Spess_t \gets \{ \s \in \mathcal{D} \mid  \\ ~~~\exists\, \s' \in \Shatp_{t-1} \colon  {l_t(\s')- L d(\s,\s') \geq 0} \}$
            \end{varwidth}
            \label{alg:goose:line:safe_set_pess}
            %
            \STATE $\Shatp_t \gets \Spess_t \cap R^{\mathrm{ergodic}}(\Spess_t, \Shatp_{t-1}) $
            \label{alg:goose:line:intersect_spess_with_ergodic}
            %
            \STATE $\Sopt_t \gets \Sopt_{t-1} \cap \{ \s \in \mathcal{D} \mid  {u_t(\s) \geq 0} \}$
            \label{alg:goose:line:safe_set_opt}
            %
            \STATE $\Shato_t \gets \Sopt_t \cap R^{\mathrm{ergodic}}(\Sopt_t,\Shato_{t-1})$
            \label{alg:goose:line:intersect_sopt_with_ergodic}
            %
            % \STATE \label{alg:goose:line:remove_unsafe_oracle_suggestion}
            % \begin{varwidth}[t]{\linewidth}
            %     \textnormal{\textbf{if}} $\s_t=\emptyset$ \textnormal{\textbf{and}} $\Shatp_t=\Shatp_{t-1}$ \\ \textnormal{\textbf{then}} $\Sopt_t \gets \Sopt_t \setminus \{\goal_k\}$, \textnormal{\textbf{go to}} \cref{alg:goose:line:oracle_suggestion}
            % \end{varwidth}
            \IF{$\s_t=\emptyset$ \textnormal{\textbf{and}} $\Shatp_t=\Shatp_{t-1}$}
                \STATE  \label{alg:goose:line:remove_unsafe_oracle_suggestion}
                $\Sopt_t \gets \Sopt_t \setminus \{\goal_k\}$, \textnormal{\textbf{go to}} \cref{alg:goose:line:oracle_suggestion}
            \ENDIF
        \ENDWHILE
        %
        \STATE Evaluate $f(\goal_k)$ and update oracle 
        \label{alg:goose:line:evaluate_suggestion}
        %
    \ENDFOR
\end{algorithmic}
\end{algorithm}
\end{minipage}
%
\hfill
%
\begin{minipage}[t]{0.46\textwidth}
\centering
\begin{algorithm}[H]
\caption{Safe Expansion (SE)}
\label{alg:SE}
\label{alg:se}
\begin{algorithmic}[1]
  \algsetup{indent=1em}
  \STATE {\bfseries Inputs:} $\Shato_t$, $\Shatp_t$, $\Spess_t$,\,$\mathcal{G}$,\,$\goal$
    %
    \STATE \label{alg:se:line:uncertain_states_W} $W_t^\epsilon \gets \{ \s \in \Shatp_t \mid u_t(\s) - l_t(\s) > \epsilon \}$
    %
    \STATE \label{alg:se:line:adjacent} 
    $\Sadj_t(p) = \{ \s \in \Shato_t \setminus \Spess_t \mid h(\s) = p \}$
    % $\Sadj_t \gets \Shato_t \setminus \Spess_t$
    %
    \STATE \label{alg:se:line:expansion_target}
    {\small // Highest priority targets in $\Sadj_t$ with expanders}
    % \begin{varwidth}[t]{\linewidth}
        $p^* \gets \max_p p \text{~~s.t.~~}  \left| g_t(W_t^\epsilon, \Sadj_t(p) ) \right| > 0$
    % \end{varwidth}
    %
    \IF{\small optimization problem feasible}
        \STATE \label{alg:se:line:expanders} 
        $G_t \gets g_t (W_t^\epsilon, \Sadj_t(p^*))$ 
        %
        \STATE \label{alg:se:line:uncertainty_sampling}
        $\s_t \gets \argmax_{\s \in G_t} \, w_t(\s)$
        %
        \STATE \label{alg:se:line:update_gp} 
        Update $\mathrm{GP}$ with $y_t = q(\s_t) + \eta_t$ 
    \ELSE
        \STATE \label{alg:se:line:emptyset}
        $\s_t \gets \emptyset$
    \ENDIF
    %
    \RETURN \label{alg:se:line:return_st}
    $\s_t$
\end{algorithmic}
%
\end{algorithm}
\end{minipage}
\end{figure*}

\paragraph{Safe expansion} 
%
%
If the oracle suggestion $\goal_k$ is not considered safe,  $\goal_k \notin \Shatp_t$, \goose employs a goal-directed scheme to evaluate a safe decision $\s_t \in \Shatp_t$ that is informative about $q(\goal_k)$, see \cref{fig:set_illustration}.
In practice, it is desirable to avoid learning about decisions beyond a certain accuracy $\epsilon$, as the number of observations required to reduce the uncertainty grows exponentially with $\epsilon$ \citep{sui2018stagewise}. Thus, we only learn about decisions in $\Shatp_t$ whose safety values are not known $\epsilon$-accurately yet in Line \ref{alg:se:line:uncertain_states_W}, $W_t^\epsilon = \{\s \in \Shatp_t \mid u_t(\s) - l_t(\s) > \epsilon\}$, where $u_t(\s) - l_t(\s)$ is the width of the confidence interval at $\s$.

To decide which decision in $W_t^\epsilon$ to learn about, we first determine a set of learning targets outside the safe set (dark blue cross in \cref{fig:set_illustration}), and then learn about them efficiently within $\Shatp_t$. To quantify how useful a learning target $\s$ is to learn about $q(\goal_k)$, we use any given iteration-dependent heuristic $h_t(\s)$. We discuss particular choices later, but a large priority $h(\s)$ indicates a relevant learning target (dashed line, \cref{fig:set_illustration}). We sort decisions that are not known to be safe or unsafe yet in $\Shato_t \setminus \Spess_t$ according to their priority in 3 and let $\Sadj_t(p)$ denote the subset of decision with equal priority.  

Ideally, we want to learn about the decisions with the highest priority. However, this may not be immediately possible by evaluating decisions within $W_t^\epsilon$. To potentially classify a decision $\z$ in $\Sadj_t(p)$ as safe, there must exist at least one decision $\s$ in $W_t^\epsilon$ that could, optimistically, attain a large enough value $q(\s)$ to determine that $\z$ is safe. We enumerate these \textit{potential expanders} through the function
$
    g_t(W_t^\epsilon, \Sadj_t(p)) = \{\s \in W_t^\epsilon, \mid \exists\, \z \in \Sadj_t(p) \colon u_t(\s) - L d(\s, \z) \geq 0 \},
$
which assumes that all decisions $\s \in W_t^\epsilon$ attain the maximum plausible value $u_t(\s)$. If this value together with the Lipschitz continuity can allow us to classify a decision $\z \in \Sadj_t(p)$ as safe, then $\s$ is a potential expander for $\Sadj_t(p)$.
%
In Line \ref{alg:se:line:expansion_target} we select the decisions with the priority level $p^*$ such that there exist uncertain, safe decisions in $W_t^\epsilon$ that could allow us to classify a decision in $\Sadj_t(p^*)$ as safe and thereby expand the current safe set $\Shatp_t$. Intuitively, we look for the highest priority targets that can potentially be classified as safe by safe evaluating decisions that we have not already learned about to $\epsilon$-accuracy.

Given these learning targets $\Sadj_t(p^*)$ (blue cross, \cref{fig:set_illustration}), we evaluate the most uncertain decision in $G_t = g_t(W_t^\epsilon, \Sadj_t(p^*))$ (blue shaded, \cref{fig:set_illustration}) in Line \ref{alg:se:line:uncertainty_sampling} and update the GP model with the corresponding observation of $q(\s_t)$ in Line \ref{alg:se:line:update_gp}. This uncertainty sampling is restricted to a small set of decisions close to the goal. This is different from methods without a heuristic that select the most uncertain secision on the boundary of $\Shatp$ (green shaded in \cref{fig:set_illustration}). In fact, our method is equivalent to the one by \citet{turchetta2016safe} when an uninformative heuristic $h(\s) = 1$ is used for all $\s$.
%
We iteratively select and evaluate decisions $\s_t$ until we either determine that $\goal_k$ is safe, or we prove that we can not safely learn about it for given accuracy $\epsilon$. In this case, we remove $\goal_k$ from the oracle's decision set in Line \ref{alg:goose:line:remove_unsafe_oracle_suggestion} of \cref{alg:goose} and query a new suggestion based on the updated safe set $\Shato_t$. 

To analyze our algorithm, we define the largest set that we can learn about as $\Rbar_\epsilon(S_0)$. This set contains all the decisions that we could certify as safe if we used a full-exploration scheme that learns the safety constraint $q$ up to $\epsilon$ accuracy for all decisions inside the current safe set. This is a natural exploration target for our safe exploration problem (see \cref{app:definitions} for a formal definition).  We have the following main result, which holds for any heuristic:
%
\begin{restatable}{theorem}{mainresult}
%Under the assumptions of~\cref{thm:beta}
Assume that $q(\cdot)$ is $L$-Lipschitz continuous w.r.t. $d(\cdot, \cdot)$ with ${\| q \|_k \leq B_q}$, $\sigma$-sub-Gaussian noise, ${S_0 \neq \emptyset}$, ${q(\s) \geq 0}$ for all~${\s \in S_0}$, and that, for any two decisions~${\s,\s' \in S_0}$, there is a path in the graph $\mathcal{G}$ connecting them within $S_0$. Let $\beta_t=B_q+4\sigma \sqrt{\gamma_t + 1 + \mathrm{ln}(1/\delta)}$, then, for any $h_t:\mathcal{D}\rightarrow \mathbb{R}$, with probability at least ${1-\delta}$, we have
%
${
q(\s)\geq \kappa
}$
%
for any $\s$ visited by~\goose.
%
Moreover, let~$t^*$ be the smallest integer such that
%
${
\frac{t^*}{\beta_{t^*}\gamma_{t^*}}\geq \frac{C\, |\overline{R}_0(S_0)|}{\epsilon^2},
}$
%
with~${C = 8 / \log(1 + \sigma^{-2})}$, then there exists a $\hat{t}\leq t^*$ such that, with probability at least~${1-\delta}$, 
%by $\hat{t}$, \cref{alg:SMDP_priority}  attains
%
$
\overline{R}_\epsilon(S_0) \subseteq \Shatp_{\hat{t}}\subseteq \overline{R}_0(S_0)$.
\label{thm:safety_and_complteness}
\end{restatable}
%
\cref{thm:safety_and_complteness} guarantees that \goose is safe with high probability. Moreover, for any priority function $h$ in \cref{alg:se}, it upper bounds the number of measurements that \cref{alg:SMDP_priority} requires to explore the largest safely reachable region $\Rbar_\epsilon(S_0)$. Note that \goose only achieves this upper bound if it is required by the \gls{IML} oracle. In particular, the following is a direct consequence of \cref{thm:safety_and_complteness}:
%
\begin{restatable}{corollary}{CorMainResult}
\label{cor:MainResult}
Under the assumptions of~\cref{thm:safety_and_complteness}, let the \gls{IML} oracle be deterministic given the observations. Then there exists a set $S$ with $\overline{R}_\epsilon(S_0) \subseteq S \subseteq \overline{R}_0(S_0)$ so that $\goal_k = \mathcal{O}(S)$ for all $k \geq 1$.
\end{restatable}
%
That is, the oracle decisions $\goal_k$ that we end up evaluating are the same as those by an oracle that was given the safe set $S$ in \cref{cor:MainResult} from the beginning. This is true since the set $\Shato_t$ converges to this set $S$. Since \cref{thm:safety_and_complteness} bounds the number of safety evaluations by $t^*$, \cref{cor:MainResult}  implies that, up to $t^*$ safety evaluations, \goose retains the properties (e.g., no-regret) of the \gls{IML} oracle $\mathcal{O}$ over $S$.

% Due to \cref{cor:MainResult}, bounds on the asymptotic cumulative unsafe regret of the oracle used by \goose easily translate to bounds on the $\epsilon$-safe average cumulative regret for \goose.
% \todo{Properly comment on regret here}

